Pareto-Optimal Fairness-Utility Amortizations in Rankings with a DBN Exposure Model

In recent years, it has become clear that rankings delivered in many areas need not only be useful to the users but also respect fairness of exposure for the item producers. We consider the problem of finding ranking policies that achieve a Pareto-optimal tradeoff between these two aspects. Several methods were proposed to solve it; for instance a popular one is to use linear programming with a Birkhoff-von Neumann decomposition. These methods, however, are based on a classical Position Based exposure Model (PBM), which assumes independence between the items (hence the exposure only depends on the rank). In many applications, this assumption is unrealistic and the community increasingly moves towards considering other models that include dependences, such as the Dynamic Bayesian Network (DBN) exposure model. For such models, computing (exact) optimal fair ranking policies remains an open question. We answer this question by leveraging a new geometrical method based on the so-called expohedron proposed recently for the PBM (Kletti et al., WSDM'22). We lay out the structure of a new geometrical object (the DBN-expohedron), and propose for it a Carath\'eodory decomposition algorithm of complexity $O(n^3)$, where $n$ is the number of documents to rank. Such an algorithm enables expressing any feasible expected exposure vector as a distribution over at most $n$ rankings; furthermore we show that we can compute the whole set of Pareto-optimal expected exposure vectors with the same complexity $O(n^3)$. Our work constitutes the first exact algorithm able to efficiently find a Pareto-optimal distribution of rankings. It is applicable to a broad range of fairness notions, including classical notions of meritocratic and demographic fairness. We empirically evaluate our method on the TREC2020 and MSLR datasets and compare it to several baselines in terms of Pareto-optimality and speed.

==> fig/sudoku_cmd.tex <==
\newcounter{row}
\newcounter{col}

\newcommand\setrow[6]{
  \setcounter{col}{1}
  \foreach \n in {#1, #2, #3, #4, #5, #6} {
    \edef\x{\value{col} - 0.5}
    \edef\y{9.5 - \value{row}}
    \node[anchor=center] at (\x, \y) {\n};
    \stepcounter{col}
  }
  \stepcounter{row}
}

==> pratenddefaultcategory.tex <==

\label{proofsection:prAtEndii}\begin{proof}[Proof of \autoref{thm:prAtEndii}]\phantomsection\label{proof:prAtEndii}The idea is to show that the scalar product \begin {equation}\label {eq:nuE} \vnu ^\top \vcE (\pi ) \end {equation} does note change whenever the ranks of two items of adjacent ranks are exchanged. All rankings can be obtained by successively exchanging the ranks of adjacent items, starting from any initial ranking. Therefore it suffices to show that \eqref {eq:nuE} remains unchanged by the exchange of the ranks of two adjacent elements. Given an arbitrary ranking $\pi _0$ the exposures of ranks $\rankix $ and $\rankix +1$ are \begin {equation} \hdots ,\underbrace {K}_{\text {rank } \rankix ,\text { item }\pi _0(\rankix )}, \underbrace {K\gamma (1-\kappa \vrho _{\pi _0(\rankix )})}_{\text {rank } \rankix +1,\text { item }\pi _0(\rankix +1)},\hdots \end {equation} for a certain constant $K$. When the items at ranks $\rankix $ and $\rankix +1$ are exchanged, to give a new ranking $\pi _1$, these exposures become \begin {equation} \hdots ,\underbrace {K}_{\text {rank }\rankix ,\text { item }\pi _0(\rankix +1)}, \underbrace {K\gamma (1-\kappa \vrho _{\pi _0(\rankix +1)})}_{\text {rank }\rankix +1,\text { item }\pi _0(\rankix )},\hdots \end {equation} while the exposures at all other ranks remain unchanged. Let us denote $i=\pi _0(\rankix )$ and $j=\pi _0(\rankix +1)$. With some algebraic manipulations, it is then easy to show that the scalar products \eqref {eq:nuE} for rankings $\pi _0$ and $\pi _1$ satisfy \begin {align} \begin {split} \vnu ^\top \vcE (\pi _1) - \vnu ^\top \vcE (\pi _0) &= \left (1+\frac {\gamma \kappa }{1-\gamma }\vrho _i\right )\left (K\gamma (1-\kappa \vrho _j) - K\right )\\ &\phantom {=}+ \left (1+\frac {\gamma \kappa }{1-\gamma }\vrho _j\right )\left (K-K\gamma (1-\kappa \vrho _i)\right )\\ &=0. \end {split} \end {align} This means that \eqref {eq:nuE} remains unchanged by exchanging two items of adjacent ranks, and thus that \eqref {eq:nuE} is constant in the whole expohedron.\end{proof}
\label{proofsection:prAtEndiii}\begin{proof}[Proof of \autoref{thm:prAtEndiii}]\phantomsection\label{proof:prAtEndiii}The proof to this theorem is quite complex, we first introduce two lemmas to build an equivalence with a well-known polytope called \emph {permutohedron}, then we show how the result can be obtained as a corollary of \cref {prop:normal}. \begin {lemm} For every $\pi \in \cS _\ndoc $, the point $\vcE (\pi ,\gamma ,\kappa ,\vrho )$ is in the zone $\zone (\pi )$. \end {lemm} \begin {proof} We need to show that \begin {equation} \vcE _{\pi (1)} \geq \hdots \geq \vcE _{\pi (\ndoc )}. \end {equation} This is clearly the case, because the exposure decreases with increasing rank. \end {proof} \begin {lemm} The vertices of the the \acrshort {dbn}-expohedron $\Pi (\gamma ,\kappa ,\vrho )$ are exactly the $\ndoc !$ points $\vcE (\pi ,\gamma ,\kappa ,\vrho )$ for $\pi \in \cS _\ndoc $. Formally \begin {equation} \vx \in \Pi (\gamma ,\kappa ,\vrho )\text { is a vertex } \iff \exists \pi \in \cS _\ndoc :~ \vx =\vcE (\pi ,\gamma ,\kappa ,\vrho ). \end {equation} \end {lemm} \begin {proof}~\\ \begin {itemize} \item "$\implies $" Every vertex of $\Pi (\gamma ,\kappa ,\vrho )$ is a point of type $\vcE (\pi ,\gamma ,\kappa ,\vrho )$, because $\Pi (\gamma ,\kappa ,\vrho )$ is the convex hull of these points. \item "$\impliedby $" To prove that a point in a polytope is a vertex, it suffices to show that it cannot be expressed as a convex combination of other vertices. Let $\pi \in \cS _\ndoc $ such that \begin {equation} \vcE (\pi ,\gamma ,\kappa ,\vrho ) = \sum _{i=1}^N \alpha _i\vcE (\pi _i,\gamma ,\kappa ,\vrho ), \end {equation} with $\sum _{i=1}^N\alpha _i=1$ and $\alpha _i>0$ for all $i\in \seq {1}{N}$. One can show by recursion over $k\in \seq {1}{\ndoc }$, that \begin {equation} \vcE _{\pi (k)}(\pi _i,\gamma ,\kappa ,\vrho ) = \vcE _{\pi (k)}(\pi ,\gamma ,\kappa ,\vrho ),~\forall i\in \seq {1}{N}. \end {equation} The highest component of $\vcE (\pi ,\gamma ,\kappa ,\vrho )$ is the number $1$ at index $\pi (1)$, so all other $\vcE (\pi _i,\gamma ,\kappa ,\vrho )$ must also have a $1$ at index $\pi (1)$. If all $\vcE (\pi _i,\gamma ,\kappa ,\vrho )$ have equal components at indices $\pi (1),\hdots ,\pi (k)$, then by the same reasoning, they must have equal components at indices $\pi (k+1)$. By recursion, they have equal indices at all components, which concludes the proof. \end {itemize} \end {proof} From previous lemmas we can conclude that $\Pi (\gamma ,\kappa ,\vrho )$ has the same combinatorial structure as the \acrshort {pbm}-expohedron \cite {kletti_introducing_2022} and as the permutohedron. Therefore a face of $\Pi (\gamma ,\kappa ,\vrho )$ is composed of vertices defined by a partial ordering of the items. Such a partial ordering can be defined by a permutation $\pi \in \cS _\ndoc $ and a set of splits $\splits \subseteq \seq {1}{\ndoc }$. Given a permutation $\pi \in \cS _\ndoc $ and a set of splits $\{s_1,\hdots ,s_N\}\subseteq \seq {1}{\ndoc }$ with $s_N=\ndoc $, the partial ordering is such that, when working in the basis of $\R ^\ndoc $ in which $\pi $ is the identity, we have \begin {equation} \vcE (\pi ')_1,\hdots ,\vcE (\pi ')_{s_1} \geq \hdots \geq \vcE (\pi ')_{s_{N-1}+1},\hdots ,\vcE (\pi ')_{s_N}, \end {equation} for every vertex $\vcE (\pi ')$ of the face. In particular, if we ignore the ranks $s_{k}+1,\hdots ,\ndoc $ for $k\in \seq {1}{N}$, we can apply \cref {prop:normal} to the ranks $s_1,\hdots ,s_{k}$ and get \begin {equation} \vnu _{s_k}=\vone (s_k)+\frac {\gamma \kappa }{1-\gamma }(\vrho \odot \vone (s_k)) \end {equation} as a normal vector to the face, which is what there was to prove.\end{proof}
\label{proofsection:prAtEndiv}\begin{proof}[Proof of \autoref{thm:prAtEndiv}]\phantomsection\label{proof:prAtEndiv}The expohedron can be partitioned into $\ndoc !$ pieces, each of which is contained by a zone. A point $\vx $ in a zone $\zone (\pi )$ is in the expohedron if and only if it is in the part of the expohedron contained by $\zone (\pi )$. Within a zone, the expohedron is delimited by $\ndoc $ hyperplanes: one hyperplane corresponds to the hyperplane of the whole expohedron (checked in line \ref {l:check_expo}) and $\ndoc -1$ other hyperplanes corespond to the $\ndoc -1$ facets adjacent to the only vertex of zone $\zone (\pi )$ (checked in line \ref {l:check_facets}). \par The determination of the zone of $\vx $ has complexity $O(\ndoc \log (\ndoc ))$. In the loop over $s\in \seq {1}{\ndoc -1}$, each scalar product has complexity $O(\ndoc )$. Therefore the complexity of the whole algorithm is $O(\ndoc ^2)$.\end{proof}
\label{proofsection:prAtEndv}\begin{proof}[Proof of \autoref{thm:prAtEndv}]\phantomsection\label{proof:prAtEndv}Once we know that a point $\vx $ is in the zone $\zone (\pi )$, it can be in at most $\ndoc -1$ facets of the expohedron at once, because there are $\ndoc -1$ facets adjacent to each unique vertex of a zone. Since every face of the expohedron is in the intersection of a certain number of facets belonging to the same zone, it suffices to check to which facets of zone $\zone (\pi )$, the point $\vx $ belongs in order to know to which faces he belongs. The lowest-dimensional such face is the one with the most normal vectors, which is what the algorithm finds. The complexity of the initial zone determination is $O(\ndoc \log (\ndoc )$, and the loop performs $\ndoc $ scalar products of vectors of size $\ndoc $, so the total complexity is $O(\ndoc ^2)$.\end{proof}
\label{proofsection:prAtEndvi}\begin{proof}[Proof of \autoref{thm:prAtEndvi}]\phantomsection\label{proof:prAtEndvi}\Cref {alg:gls} implements the \acrshort {gls}, which is proven to yield the Carathéodory decomposition of any point inside the polytope on which it is applied \cite {grotschel_geometric_1993}. The most complex operation in the loop has complexity $O(\ndoc ^2)$ so the total complexity of the algorithm is $O(\ndoc ^3)$.\end{proof}
\label{proofsection:prAtEndvii}\begin{proof}[Proof of \autoref{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}The fact that the algorithm builds the Pareto front is sufficiently explained in the paragraph preceding the pseudo-code. The complexity of the most complex operation inside the loop is $O(\ndoc ^2)$ and the loop has length at most $\ndoc $, so the total complexity of the algorithm is $O(\ndoc ^3)$.\end{proof}


==> tikzlibraryrightangles.code.tex <==
% Copyright 2013 by Till Tantau
% Copyright 2018 by Kpym T.
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: https://github.com/kpym/tikz-rightangles/blob/master/tikzlibraryrightangles.code.tex,v 1.0 2018/01/09 kpym$


\tikzset{
  pics/right angle/.style = {
    setup code  = \tikz@lib@angle@parse#1\pgf@stop,
    background code = \tikz@lib@rightangle@background#1\pgf@stop,
    foreground code = \tikz@lib@rightangle@foreground#1\pgf@stop,
  },
  pics/right angle/.default=A--B--C,
  angle eccentricity/.initial=.6,
  angle radius/.initial=5mm
}

\def\tikz@lib@rightangle@background#1--#2--#3\pgf@stop{%
  \path [name prefix ..] [pic actions, draw=none] (#2.center)
    -- ++(\tikz@start@angle@temp:\tikz@lib@angle@rad pt)
    -- ++(\tikz@end@angle@temp:\tikz@lib@angle@rad pt)
    -- ++(\tikz@start@angle@temp:-\tikz@lib@angle@rad pt)
    -- cycle;
}

\def\tikz@lib@rightangle@foreground#1--#2--#3\pgf@stop{%
  \path [name prefix ..] [pic actions, fill=none, shade=none]
  ([shift={(\tikz@start@angle@temp:\tikz@lib@angle@rad pt)}]#2.center)
  -- ++(\tikz@end@angle@temp:\tikz@lib@angle@rad pt)
  -- ++(\tikz@start@angle@temp:-\tikz@lib@angle@rad pt);
  \ifx\tikzpictext\relax\else%
    \def\pgf@temp{\node()[name prefix
      ..,at={([shift={({.5*\tikz@start@angle@temp+.5*\tikz@end@angle@temp}:\pgfkeysvalueof{/tikz/angle
            eccentricity}*0.707107*\tikz@lib@angle@rad pt)}]#2.center)}]}% sqrt(1/2) = 0.7071067811865476
    \expandafter\pgf@temp\expandafter[\tikzpictextoptions]{\tikzpictext};%
  \fi
}


\def\tikz@lib@angle@parse#1--#2--#3\pgf@stop{%
  % Compute radius:
  \pgfmathsetmacro\tikz@lib@angle@rad{\pgfkeysvalueof{/tikz/angle radius}}
  \ifdim\tikz@lib@angle@rad pt>0pt\else\def\tikz@lib@angle@rad{12}\fi%
  % Compute first coordinate:
  \pgf@process{\pgfpointanchor{#2}{center}}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgf@process{\pgfpointanchor{#1}{center}}%
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  \pgf@process{\pgfpointanchor{#3}{center}}%
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  \advance\pgf@xb by-\pgf@xa%
  \advance\pgf@yb by-\pgf@ya%
  \advance\pgf@xc by-\pgf@xa%
  \advance\pgf@yc by-\pgf@ya%
  \pgfmathsetmacro{\tikz@start@angle@temp}{atan2(\the\pgf@yb,\the\pgf@xb)}
  \pgfmathsetmacro{\tikz@end@angle@temp}{atan2(\the\pgf@yc,\the\pgf@xc)}
  \ifdim\tikz@end@angle@temp pt<\tikz@start@angle@temp pt%
    \pgfmathsetmacro{\tikz@start@angle@temp}{\tikz@start@angle@temp-360}%
  \fi%
}



\endinput

